BARISTA: Efficient and Scalable Serverless Serving System for Deep Learning Prediction Services

Pre-trained deep learning models are increasingly being used to offer a variety of compute-intensive predictive analytics services such as fitness tracking, speech and image recognition. The stateless and highly parallelizable nature of deep learning models makes them well-suited for serverless computing paradigm. However, making effective resource management decisions for these services is a hard problem due to the dynamic workloads and diverse set of available resource configurations that have their deployment and management costs. To address these challenges, we present a distributed and scalable deep-learning prediction serving system called Barista and make the following contributions. First, we present a fast and effective methodology for forecasting workloads by identifying various trends. Second, we formulate an optimization problem to minimize the total cost incurred while ensuring bounded prediction latency with reasonable accuracy. Third, we propose an efficient heuristic to identify suitable compute resource configurations. Fourth, we propose an intelligent agent to allocate and manage the compute resources by horizontal and vertical scaling to maintain the required prediction latency. Finally, using representative real-world workloads for urban transportation service, we demonstrate and validate the capabilities of Barista.

==> future.tex <==
% $Id$
By surveying the literature in Section~\ref{sec:survey}, we find
some gap needs to filled for automatic transformation of the
business-relevant model to TOSCA-compliant deployable model. First, we
need to define a metamodel for the business user, who makes the model
on top of that without the need to be a domain expert.  The metamodel
will then transform the user model to TOSCA-compliant deployable model
in an efficient and optimal way and will also guarantee the
correctness of the model. The Aeolus project approach is a good
solution to reach the goal, but it did not build on top of TOSCA
specification which is a standard.  On the other hand, OpenTOSCA
approach is TOSCA-compliant, but it lacks the robustness of the CSP
solver. 

We built the metamodel for the business user using a web version of
GME (Generic Modeling Environment)
toolkit~\cite{ledeczi2001generic}. It is a toolkit for creating a
Domain Specific Modeling Language (DSML) through metamodel specifying
the modeling language of the application domain. In the modeling
language, we specified all the syntactic, semantic, and presentation
information regarding the domain, which needs to be used to construct
deployable models using ansible.  We created the model for this
transformation in webGME, which will be the metamodel for the
users. We provided specific interpreters for our WebGME model, which
convert any user-defined model to a TOSCA-compliant Ansible deployable
model.   

In future, our DSML generated ansible script needs to be verified
using a CSP solver, and it will prove its soundness and robustness. We
would also like to add type-based and AI-based pattern matching
approach for finding software dependencies, and we can make our DSML
learn from the history by using machine-learning techniques.  The
migration of application components is also a necessary feature
which needs to be automated. 


==> problem.tex <==
% $Id: problem.tex 35953 2018-05-19 07:02:13Z chhokraad $
%----------------------------------------------------------------------
This section uses real-world use cases to formulate the problem that
we solve in this paper. 
\iffalse
% this is repetitive
In section~\ref{sec:introduction}, we
briefly introduced the requirements to guarantee QoS for the
predictive analytics services that are based on deep machine learning
trained models, and in this section, we elaborate on these
requirements. 

%
Predictive analytics based on deep machine learning trained models are
published as services such as voice recognition services (Amazon
Alexa, Apple Siri, etc.), image recognition services(e.g., Google
Translator, etc.) and many more. For example, automatic speech
recognition and subtitle generation for live video streaming require
to run a pre-trained model in the backend, and whenever speech is
detected, it should be transcribed and displayed as text.  Multiple
videos can be broadcasted at the same time on an eventful day to
numerous subscribers, who require subtitles. Users submit their
requests using interactive web API or mobile applications and expect
the predicted results back within seconds. The response time should be
within specific SLA bound; otherwise, the service providers will be
penalized by loss of users and other forms of monetary loss. To
account for the profitability aspects of the service providers, they
do not want to over-provision the system, and the service providers
want to minimize the dedicated resources while guaranteeing the
QoS. To strategize for the optimal resource allocation while ensuring
the QoS, we need to address the below challenges.   

\paragraph{\textbf{\textit{\large Requirements: }}} 
\fi
Specifically we focus on categorizing and solving challenges regarding the influence on the performance of Deep Machine Learning Prediction Services deployed on container platforms.  We assume that containers are allocated inside virtual machines (VMs).  Our primary goal is to design a deployment and management platform to guarantee the SLOs for deep machine learning-based prediction services hosted using serverless computing.  We investigate latency and performance implications related to infrastructure elasticity, vertical scaling of resources dynamically, load balancing, workload variation prediction and resource interference.  In this context, we formulate the following key requirements for our solution.

\subsection{\large R1: Accounting for the Implication of Infrastructure Elasticity}

\label{sec:R1}
For deployment of new services and to perform horizontal
scaling~\cite{lorido2014review}, service infrastructure must be
provisioned pro-actively or re-actively to respond to the client
requests within SLO bounds.  The virtualized cloud infrastructure can
be in four states:  (1) VM Cold, (2) Container Cold, (3) Container
Warm and (4) Container Running. 
\begin{enumerate}
\item \textit{VM Cold} means that the
virtual machines need to be started to handle new client
requests. 
\item \textit{Container Cold} means containers need to be
provisioned in the VM to handle new client requests. 
\item \textit{Container
  Warm} means Docker containers need to be run to load the pre-trained
model in the container's memory to handle new client requests, and
\item \textit{Container Running} means the Docker containers need to run
the prediction service to provide the result for the new client
requests.  
\end{enumerate}
Therefore, each state in the reverse direction, i.e., 4$\rightarrow$1 incurs an additional delay in processing the requests.  Pre-trained deep learning prediction models are large.  Hence, the load time of these models takes a significant amount of time.  In our work, we studied how the response times will be impacted in the current infrastructure states, and this impact is accounted for in minimizing the SLO misses while avoiding excess over-provisioning and longer retention of unused infrastructure.

\begin{figure}[htb]
	
	\centering
	\includegraphics[width=\linewidth]{images/modelspwanTime.png}
	\caption{The prediction service deployment time for different deep learning model is shown here. The blue bar is the worst case time (as per our experiment) to spawn a VM, orange bar shows the download time of specific container, and grey bar shows the loading time of the model. }
	\label{Fig:modelspwanTime}
\end{figure}

In this paper, we refer to the VM Cold state as the $t_{vm}$ time, which is the combination of time to spawn VM, download the containerized service (`container cold' state, i.e., $t_{cc}$), and load the pre-trained model (`container warm' state, i.e., $t_{w}$) in memory to run it.  The deployment times for each infrastructure state for different prediction services is shown in Figure~\ref{Fig:modelspwanTime}.  This motivates the need to forecast the future workload $t_{vm}$ timestamps ahead to guarantee the SLO, and we will check the infrastructure state in $t_{cc}$ and $t_{w}$ timestamps ahead to take decisions for downloading and starting the containerized service if it is not already in running state. We need to predict on different forecasting window size because $t_{vm}$ time of different deep learning prediction model varies. 

\subsection{\large R2: Selecting Optimal Number of Resources and Auto Scaling} 
\label{sec:R2}
Selecting an optimal number of virtual machines from the cloud provider is
required to optimize the cost~\cite{yadwadkar2017selecting}.  Deep
learning prediction models are very compute-intensive and can run
faster if more cores are allocated.  In Figure~\ref{Fig:modeltime}, we
have benchmarked the prediction times for several deep learning
pre-trained models (containerized) on a \textit{Intel(R) Xeon(R) CPU
  E5-2640 v4} bare-metal machine by varying the number of assigned CPU
cores.  We performed ten thousand trial executions to benchmark the
models on the same bare-metal machine.  It is clear from the figure
that the pre-trained models can be parallelized due to which
prediction times can be reduced if more CPU cores can be assigned to
these models. 

\begin{figure*}[hbt]
	\centering
	%    \includegraphics[width=6.5in]{images/plan.png}
	\includegraphics[width=\textwidth]{images/modeltime.png}
	\caption{Box plot of prediction time of different large deep learning (VGG19, InceptionResnetV2, ResNet50, DenseNet, InceptionV3, Xception, Google Word2Vec) pre-trained model on different number of cpu cores(2,4 and 8)}
	\label{Fig:modeltime}
\end{figure*}

Thus, selecting VMs with more cores is beneficial, but this must be done accounting for the cost too.  Our goal is to choose the optimal VM, which can meet the SLO of the prediction while minimizing cost. In this context, vertical elasticity is attractive because it has the ability to dynamically resize resources for the applications residing in containers or virtual machines~\cite{al2018coordinating,lakew2014towards}. It allows fine-grained assignment of resources to the application to meet its resource demands at runtime.  Dynamic vertical resource elasticity is faster than attempting horizontal scaling.  The downside is that it is only applicable if the service infrastructure is in the \textit{Container Running} state, and the required resources are available in the virtual machine.  In the \textit{Container Running} state, the container can be in the idle state or the busy state.  We explore this area to find if using vertical scaling we can deallocate and allocate some cores, which can be used for other batch running services on the VM.   

\subsection{\large R3: Load Balancing }
\label{sec:R3}
% Anirban, I don't see a requirement coming out in this but rather
% just a statement of what we are going to do.
Cloud and service providers typically perform load balancing based on
CPU load or in a round-robin fashion to distribute the incoming client
requests among the available backend servers or virtual
machines~\cite{lloydserverless}.  Rather than attempting the load
balancing in a reactive and centralized manner, in this paper, we
present a de-centralized and proactive approach to handle the incoming
load based on time-series prediction analysis and forecasting of
application performance.  Requests wait in the front end of the
service to receive the result back within a timeout period, and if
there is a network problem, it will receive an exception.  As the
services are stateless, there is no need to provide any consensus
algorithm using message queuing and message brokers.  However, any of
these additional capabilities can be easily integrated with the
current architecture of BARISTA.

% Might need to change
\subsection{\large R4: Workload Forecasting}
\label{sec:R4}
Proactive, dynamic provisioning of resources can be achieved by
forecasting future demands of applications based on historical time
series usage pattern for that application. Many techniques exist for
forecasting. The \emph{Prophet Forecasting} model is becoming increasingly adopted by industries for efficient and fast prediction of resource utilization    with minimal impact on the QoS. In this paper, we uses Prophet for the above mentioned reasons.


%The \emph{Autoregressive integrated moving average
%  (ARIMA}) model is used widely in the
%literature~\cite{calheiros2015workload,	roy2011efficient} for
%efficient prediction of resource utilization with minimal impact on
%the QoS.  In this paper, we also consider ARIMA model for our online
%workload forecasting.

\subsection{\large R5: Awareness to Performance Interference} 
\label{sec:R5} 
By co-locating various application models on a number of servers can host a significant amount of workload and provide better scalability while minimizing the resource usage. Despite all these advances in vertical elasticity techniques, performance interference between the co-scheduled application models on a single server or virtual machine can adversely impact SLOs of the applications~\cite{nathuji2010q,delimitrou2013paragon,delimitrou2014quasar}. Hence, these challenges necessitate a solution approach to be performance interference aware in the worst-case scenario due to co-location of the application models. To support our claim in the context of prediction models, in Figure~\ref{Fig:contention} we portray the prediction time of deep learning Xception pre-trained model on four CPU cores in isolation, and along with large Google Word2Vec deep learning pre-trained model on four other CPU cores (blue)  in an eight cores VM.  The Google Word2Vec model is a large model where the container uses 7.8GB of memory and 4 CPU cores. Performance degradation is approximately 16\% for Xception model's prediction time stemming primarily from performance interference.  Thus, resource allocations schemes need to aware of performance interferences.  In our approach, we allow 20\% performance degradation (for the worst-case scenario) due to performance interference.

\begin{figure}[htb]
	\centering
	%    \includegraphics[width=6.5in]{images/plan.png}
	\includegraphics[width=\linewidth]{images/contention.png}
	\caption{Prediction time plot of deep learning Xception pre-trained model on 4 cpu cores in isolation(red) and along with large Google Word2Vec deep learning pre-trained model on 4 other cpu cores(blue) in a 8 cores VM. Performance degradation is approximately 16\% for Xception model. }
	\label{Fig:contention}
\end{figure}


